$\phi$-Decoding: Adaptive Foresight Sampling for Balanced Inference-Time Exploration and Exploitation

Inference-time optimization scales computation to derive deliberate reasoning steps for effective performance. While previous search-based strategies address the short-sightedness of auto-regressive generation, the vast search space leads to excessive exploration and insufficient exploitation. To strike an efficient balance to derive the optimal step, we frame the decoding strategy as foresight sampling, leveraging simulated future steps to obtain globally optimal step estimation. Built on it, we propose a novel decoding strategy, named $\phi$-Decoding. To provide a precise and expressive estimation of step value, $\phi$-Decoding approximates two distributions via foresight and clustering. Sampling from the joint distribution, the optimal steps can be selected for exploitation. To support adaptive computation allocation, we propose in-width and in-depth pruning strategies, featuring a light-weight solution to achieve inference efficiency. Extensive experiments across seven benchmarks show $\phi$-Decoding outperforms strong baselines in both performance and efficiency. Additional analysis demonstrates its generalization across various LLMs and scalability across a wide range of computing budgets. The code will be released at https://github.com/xufangzhi/phi-Decoding, and the open-source PyPI package is coming soon.

==> sections/1.introduction.tex <==
\section{Introduction}

Large language models (LLMs)~\cite{achiam2023gpt, team2023gemini} present remarkable performances in solving reasoning-intensive tasks through step-by-step thoughts~\cite{wei2022chain}.
Recent advancements, like o1 and QwQ~\cite{qwq-32b-preview}, have significantly bolstered LLM reasoning by post-training on well-curated long-form chain-of-thought datasets.
Nevertheless, the huge cost associated with the post-training procedure hinders its reproducibility. \changh{Not sure post-training has huge cost, maybe change to:}\chang{Recent result show that inference-time strategy could be superior for optimizing LLM reasoning at a lower cost \citep{}}
This naturally motivates us to delve into the inference-time strategy for optimizing the LLM reasoning chains.

\changh{Generally the first part of this paragraph is unclear: why autoregressive is not good enough, and why foresight is needed is not clear.}\chang{Inference-time strategies utilize more reasoning tokens that encodes thinking steps to perform effective reasoning. However, the natural short-sightedness of autoregressive generation makes most inference algorithms unable to adhere to long-term goals~\cite{ma2024non}. Most previous work solve this by deliberately optimizing each step using search-based methods~\citep{yao2024tree, hao2023reasoning, xie2024self,wu2024inference}, the exploration and backtracking of tree search algorithms enable LLMs to find global-optimal reasoning paths. Nevertheless, these approaches often entail extensive time costs or yield in adequate assessments of step values. In contrast, if we could have a precise estimation of global-aware step values, less exploration is necessary and could improve the efficiency of reasoning~\citep{wang2024math, ma2024non}. Therefore, to strike an efficient balance between inference-time exploration and exploitation, it is inevitable to obtain reliable and expressive step value estimations.}
Central to this process is the critical task of estimating the values.
Previous work, Guided Decoding~\cite{xie2024self}, utilizes stepwise self-evaluation to calibrate the reasoning, which ignores the inherent limitations of auto-regressive generation.\changh{Guided decoding uses beam search, so it's already improving autoregressive generation. Delete this example perhaps, and move the citation to search.} 
% Due to the inherent limitations of auto-regressive generation, producing reliable and optimal intermediate steps presents significant hurdles. 
The decision-making process of the LLMs for each subsequent step relies solely on preceding steps, resulting in a lack of foresight~\cite{ma2024non}.
Fig.X(a) presents the notable disparities \changh{Need to give a more detailed explanation of the disparity}that arise between the model confidence at individual steps and both (i) the final accuracy and (ii) the model confidence across completed reasoning paths. \xfz{pilot exp}
% To address this limitation, prior searching-based methods~\cite{yao2024tree,hao2023reasoning} attempt to select the optimal step via tree search,
% which involves extensive time costs for expanding and backtracking.
% Considering the efficiency, the sampling-based method~\cite{ma2024non} proposes to find non-myopic steps sequentially by looking ahead.
To address this limitation, prior searching-based~\cite{yao2024tree,hao2023reasoning} and sampling-based methods~\cite{ma2024non} derive step values through backtracking and foresight sampling techniques, respectively. Nevertheless, these approaches often entail extensive time costs or yield inadequate assessments of step values.
From Fig.X(b), both of the methods fail to fill the obvious distribution gaps between the estimated step values and the final answer.
\xfz{pilot exp}
It leaves a huge blank to
(1) \emph{obtain the reliable and expressive step value} and
(2) \emph{strike the balance between inference-time exploration and exploitation}.

% However, it primarily exploits the most optimal previous steps without ensuring diversity via exploration.
% However, it solely bases the step value on the model confidence of the foresight paths.
% Built upon these initial attempts,
% our paper addresses the following two critical questions:
% (1) \emph{How to obtain the reliable step value estimation?}
% (2) \emph{Does every step require deliberation for decision-making?}

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.62]{Figures/intro_step_value.pdf}
    \vspace{-0.2cm}
    \caption{Step value analysis.}
    \label{fig:sub1}
  \end{subfigure}
  % \\
  % \begin{subfigure}{0.5\textwidth}
  %   \centering
  %   \includegraphics[scale=0.62]{Figures/intro_step_value.pdf}
  %   \vspace{-0.2cm}
  %   \caption{Base LLM: Qwen2.5-7B-Instruct}
  %   \label{fig:sub2}
  % \end{subfigure}
  \caption{Pilot experiments.}
  \label{fig:pilot}
\end{figure}

\changh{I feel that somehow both points could be surrounding: striking the balance between inference-time exploration and exploitation: 1) good values estimation needs less exploration and could be more efficient and effective 2) place more workload to estimate crucial step values. Maybe could mention the topic repeatedly during writing, to make the paper more centered and solves a single important question.}
\chang{Another issue of stepwise optimization is whether} \emph{ every step requires deliberation for decision-making.}
Naturally, more computational resources should be allocated to challenging steps, while conserving compute for simpler steps.
Fig.X(c) gives a pilot observation that cutting xxx \% of thinking computation would only lead to xxx\% performance drops.\xfz{pilot exp}
The previous inference-time optimization methods widely overlook this principle.
In addition, such concept of \emph{over-thinking} has been widely observed in the o1-like attempts~\cite{chen2024not}.
% However, few efforts have been made to alleviate the unnecessary compute.
Therefore, it is both intriguing and promising to develop a solution that \chang{adaptively balances} computational workload.

In this paper, we propose a novel inference-time optimization algorithm \ours, which introduces an adaptive foresight sampling strategy to perform non-myopic \changh{I think this notion is not introduced before} reasoning with alleviated over-thinking.
To give the reliable and expressive step value estimation, 
\ours capitalizes on foresight paths to derive two distributions: one from step \emph{advantage} values \changh{introduce advantage} , capturing uncertainty discrepancies between successive steps, and another from syntax-level clustering of these foresight paths. Sampling from the joint distribution, \ours selects optimal steps.
To address the challenge of overthinking,
\ours introduces the width and depth pruning strategies purely with LLM self-evaluation,
which provides adaptive inference-time scaling.
On diverse reasoning benchmarks,
\ours improves the average performance of LLaMA3.1-Instruct-8B by 11\% over auto-regressive CoT.
Compared with previous searching-based and sampling-based baselines,
\ours offers a superior balance between performance (Accuracy) and computational efficiency (\#FLOPS). We also provide insightful \changh{be more specific, and mention conclusions here} analyses of \ours's generalizability to other backbone LLMs and the underlying reasons for its superiority.

The major contributions of our work are:

\noindent (1) \textbf{An inference-time optimization algorithm \ours without external auxiliary}. \ours estimates the step value based on the joint distribution derived from foresight paths. Width and depth pruning strategies are introduced to alleviate the overthinking issue.

\noindent (2) \textbf{Comprehensive experiments with superior performances.}
\ours improves the average reasoning of LLaMA3.1-8B-Instruct by 12\%, presenting a great trade-off between effectiveness and efficiency compared with baselines.
Its generalizability to other backbone LLMs is well verified.

\noindent (3) \textbf{Insightful findings and discussions.}\changh{This title of this point should be more specific, like mentioning the most key insightful finding}
Our research also provides valuable insights into the underlying reasons for superiority as well as the scaling of inference-time computing,
paving the way for future research.


